Capacity: Cryptographically-Enforced In-Process Capabilities for Modern ARM Architectures (Extended Version)

In-process compartmentalization and access control have been actively explored to provide in-place and efficient isolation of in-process security domains. Many works have proposed compartmentalization schemes that leverage hardware features, most notably using the new page-based memory isolation feature called Protection Keys for Userspace (PKU) on x86. Unfortunately, the modern ARM architecture does not have an equivalent feature. Instead, newer ARM architectures introduced Pointer Authentication (PA) and Memory Tagging Extension (MTE), adapting the reference validation model for memory safety and runtime exploit mitigation. We argue that those features have been underexplored in the context of compartmentalization and that they can be retrofitted to implement a capability-based in-process access control scheme. This paper presents Capacity, a novel hardware-assisted intra-process access control design that embraces capability-based security principles. Capacity coherently incorporates the new hardware security features on ARM that already exhibit inherent characteristics of capability. It supports the life-cycle protection of the domain's sensitive objects -- starting from their import from the file system to their place in memory. With intra-process domains authenticated with unique PA keys, Capacity transforms file descriptors and memory pointers into cryptographically-authenticated references and completely mediates reference usage with its program instrumentation framework and an efficient system call monitor. We evaluate our Capacity-enabled NGINX web server prototype and other common applications in which sensitive resources are isolated into different domains. Our evaluation shows that Capacity incurs a low-performance overhead of approximately 17% for the single-threaded and 13.54% for the multi-threaded webserver.

==> Makefile <==
# Latex Makefile using latexmk
# Modified by Dogukan Cagatay <dcagatay@gmail.com>
# Originally from : http://tex.stackexchange.com/a/40759
#
# Change only the variable below to the name of the main tex file.
PROJNAME=$(shell basename $(CURDIR))


# You want latexmk to *always* run, because make does not have all the info.
# Also, include non-file targets in .PHONY so they are run regardless of any
# file of the given name existing.
.PHONY: $(PROJNAME).pdf all clean

# The first rule in a Makefile is the one executed by default ("make"). It
# should always be the "all" rule, so that "make" and "make all" are identical.
all: $(PROJNAME).pdf

# CUSTOM BUILD RULES

# In case you didn't know, '$@' is a variable holding the name of the target,
# and '$<' is a variable holding the (first) dependency of a rule.
# "raw2tex" and "dat2tex" are just placeholders for whatever custom steps
# you might have.

%.tex: %.raw
	./raw2tex $< > $@

%.tex: %.dat
	./dat2tex $< > $@

# MAIN LATEXMK RULE

# -pdf tells latexmk to generate PDF directly (instead of DVI).
# -pdflatex="" tells latexmk to call a specific backend with specific options.
# -use-make tells latexmk to call make for generating missing files.

# -interactive=nonstopmode keeps the pdflatex backend from stopping at a
# missing file reference and interactively asking you for an alternative.

PDFLATEX_OPT="pdflatex -synctex=1 -interaction=nonstopmode -file-line-error"

$(PROJNAME).pdf: main.tex
	latexmk  --jobname=$(PROJNAME) -pdf \
	-pdflatex=$(PDFLATEX_OPT) -use-make $<

cleanall:
	rm -rf *.aux *.bbl *.blg *.fdb_latexmk  \
	*.fls *.log *.out

clean:
	rm -rf *.aux *.bbl *.blg *.fdb_latexmk  \
	*.fls *.log *.out *.synctex.gz



==> listings/backup <==
  ...
// /*!\textcolor{clr-comment}{\tt Dom$_{curr}$ $=$ Dom$_{enc}$ }!*/, /*!\textcolor{clr-comment}{\tt \key{DB} $=$ \key{Dom_{enc}} } !*/
  capac_enter(DOM_ENCRYPT); 
  encrypt(/*!\hlgray{plaintext}!*/, /*!\hlgray{ciphertext}!*/, sz);
  capac_exit();
  ...
void encrypt (const char** /*!\hlgray{plaintext}!*/,
              char** /*!\hlgray{ciphertext}!*/, 
              int size) {
// Refmon authenticates path then returns signed FD
  int /*!\hlblue{fd}!*/; /*!\hfill\action{FD-Sign}!*/      /*!\label{line:fd-sign}!*/
    = open(/*!\hlblue{"secret\_key.txt"}!*/, /*!\hfill\action{Path-Auth}!*/ /*!\label{line:path-auth}!*/
            O_RDONLY); 

// capac_malloc() allocates tagged memory and returns tagged PTR
  DOM_PRIV_PTR char* /*!\hlblue{secret\_key}!*/ /*!\hfill\action{PTR+MEM-Tag}!*/  
      = capac_malloc(size); /*!\label{line:ptr-sign}!*/
// Ref. monitor authenticates fd in sys_read
  read (/*!\hlblue{fd}!*/, /*!\hlblue{secret\_key}!*/); /*!\hfill\action{FD-Auth}!*/ /*!\label{line:fd-auth}!*/
  for (int i = 0; i < size; i++)
      /*!\hlgray{*ciphertext}!*/[i] 
          // signed ptr is authenticated before use
      = /*!\hlblue{secret\_key}!*/[i] ^ /*!\hlgray{*plaintext}!*/[i]; /*!\hfill\action{PTR-Auth}!*/ /*!\label{line:ptr-auth}!*/
}
/*!
\begin{flushleft}
{\sffamily \footnotesize
\noindent\hlblue{\ \ \ \ \ \ \ \ } : Domain-private objects
\\
\hlgray{\ \ \ \ \ \ \ \ } : Ambient objects
\\
\action{Action} : \thename's actions 
}
\end{flushleft}
!*/

==> listings/capacity-action-figure.bak.tex <==
\tcbset{listing engine=listings}



\begin{figure*}[t]
\begin{minipage}[t]{.36\textwidth}
\begin{lstlisting}[style=sslab-mini-c,linewidth=7.2cm]
  ...
// /*!\textcolor{clr-comment}{\tt Dom$_{curr}$ $=$ Dom$_{enc}$ }!*/, /*!\textcolor{clr-comment}{\tt \key{DB} $=$ \key{Dom_{enc}} } !*/
  capac_enter(DOM_ENCRYPT); /*!\hfill\action{DomainEntry}!*/ 
  encrypt(/*!\hlgray{plaintext}!*/, /*!\hlgray{ciphertext}!*/, sz);
  capac_exit();
  ...
void encrypt (const char** /*!\hlgray{plaintext}!*/,
              char** /*!\hlgray{ciphertext}!*/, 
              int size) {
  DOM_PRIV_PTR char** /*!\hlblue{secret\_key}!*/
  // ref. mon. authenticates path then returns signed FD
  int /*!\hlblue{fd}!*/;   /*!\label{line:fd-sign}!*/ /*!\hfill\action{FD-Sign}!*/      

            = open(/*!\hlblue{"secret\_key.txt"}!*/,   /*!\label{line:path-auth}!*/ /*!\hfill\action{PATH-Auth}!*/ 
     
          O_RDONLY); 

// capac_malloc() allocates tagged memory and returns tagged PTR
  DOM_PRIV_PTR char** /*!\hlblue{secret\_key}!*/ /*!\hfill\action{PTR-Sign}!*/  
            = capac_malloc(size); /*!\label{line:ptr-sign}!*/  /*!\hfill\action{PrivMemAlloc}!*/
// Ref. monitor authenticates fd in sys_read
  read (/*!\hlblue{fd}!*/, /*!\hlblue{secret\_key}!*/); /*!\label{line:fd-auth}!*/ /*!\hfill\action{FD-Auth}!*/
  
  for (int i = 0; i < size; i++)
    /*!\hlgray{*ciphertext}!*/[i] 
    // signed ptr is authenticated before use
    = /*!\hlblue{secret\_key}!*/[i] ^ /*!\hlgray{*plaintext}!*/[i]; /*!\label{line:ptr-auth}!*/ /*!\hfill\action{PTR-Auth}!*/
    
}
/*!
\begin{flushleft}
{\sffamily \footnotesize
\noindent\hlblue{\ \ \ \ \ \ \ \ } : Domain-private objects
\\
\hlgray{\ \ \ \ \ \ \ \ } : Ambient objects
\\
\action{Action} : \thename's actions 
}
\end{flushleft}
!*/
\end{lstlisting}
\end{minipage}
\hfill
\begin{minipage}[t]{.5\textwidth}
\begin{minipage}[t]{.40\textwidth}
\begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{green!20},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,framexrightmargin=1pt,belowskip=1pt ,name=entrylib]
entry_token_t token = pacga(target_dom);
domain_switch_ioctl(token);
\end{lstlisting}
\end{minipage} 
\hspace{11pt}
\begin{minipage}[t]{.5\textwidth}
\begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{ssblue!20},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt, name=entrykernel]
dom_id_t target_dom = authenticate_entry(token);
switch_domain_key(target_dom);
\end{lstlisting}
\end{minipage} 
\begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{ssblue!20},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt, name=pathauth]
authenticate_path("secret_key.txt", kernel_secret);
int raw_fd = open("secret_key.txt", O_RDONLY);
return sign_fd(raw_fd, kernel_secret);
\end{lstlisting}



\begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{ssblue!20},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt, name=fdauth]
int raw_fd = authenticate_fd(fd, kernel_secret);
return read(raw_fd);
\end{lstlisting}

 
\begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{green!20},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt, name=memalloc]
domain_signature_t dom_sig = DST[curr_dom];
int tag_num = authenticate_signature(dom_sig);
return allocate_tagged_mem(size, tag_num);
\end{lstlisting}

\begin{lstlisting}[style=sslab-mini-c,language={[ARM]Assembler},keepspaces,numbers=none,backgroundcolor=\color{red!20},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt,name=domptrsign]
pacdzb  x0	        // Sign domain-priv. PTR with dom. key
str	    x0, [x25]   // Store PTR into memory
\end{lstlisting}
\begin{lstlisting}[style=sslab-mini-c,language={[ARM]Assembler},keepspaces,numbers=none,backgroundcolor=\color{red!20},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt,name=domptrauth]
ldr     x13, [x25]  // Load domain-priv. PTR from memory
autdzb  x13         // Authenticate with dom. key 
\end{lstlisting}
\begin{lstlisting}[style=sslab-mini-c,language={[ARM]Assembler},keepspaces,numbers=none,backgroundcolor=\color{red!20},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt, name=ambptrauth]
ldr     x13, [x1]    // Load ambient PTR from memory
autdza  x12          // Authenticate with ambient key
\end{lstlisting}
\end{minipage}
\begin{tikzpicture}[
  remember picture,
  overlay,
  annotation/.style={
    inner sep=0pt,
    outer sep=0pt,
    outer xsep=1mm,
    text width=5cm
  },
%   >={Stealth[inset=0pt, angle=45:7pt]}
]
\draw (pic cs:line-pathauth-1-start) node[annotation, above, yshift=1.6ex,xshift=3cm]{\action{PATH-Auth+FD-Sign}};
\draw (pic cs:line-fdauth-1-start) node[annotation, above, yshift=1.6ex,xshift=3cm]{\action{FD-Auth}};
\draw (pic cs:line-domptrauth-1-start) node[annotation, above, yshift=1.6ex,xshift=3cm]{\action{FD-Auth}};
\draw (pic cs:line-entrylib-1-start) node[annotation, above, yshift=1.6ex,xshift=3cm]{\action{DomainEntry}};
\draw (pic cs:line-entrykernel-1-start) node[annotation, above, yshift=1.6ex,xshift=3cm]{\action{DomainEntry}};
\draw (pic cs:line-domptrsign-1-start) node[annotation, above, yshift=1.6ex,xshift=3cm]{\action{PTR-Sign (Dom-Priv)}};
\draw (pic cs:line-domptrauth-1-start) node[annotation, above, yshift=1.6ex,xshift=3cm]{\action{PTR-Auth (Dom-Priv)}};
\draw (pic cs:line-ambptrauth-1-start) node[annotation, above, yshift=1.6ex,xshift=3cm]{\action{PTR-Auth (Ambient)}};
\end{tikzpicture}

\caption{\thename's domain-private objects and \thename's actions that enforce their isolation.}
\label{fig:code-example}
\end{figure*}

==> listings/capacity-action-figure.tex <==
\begin{figure*}[t]
\begin{minipage}[t]{.43\textwidth}
\begin{lstlisting}[style=sslab-mini-c,linewidth=.9\textwidth,name=codeexample]
typedef struct encrypt_context {
  char *secret_key;
} encrypt_context_t;
...
  capac_enter(DOM_ENCRYPT);
  read_secret_key(/*!\hlblue{ctx}!*/);
  encrypt(/*!\hlblue{ctx}!*/, /*!\hlgray{plaintext}!*/, /*!\hlgray{plaintext}!*/, size);
  capac_exit();
...
void read_secret_key(
        DOM_PRIV encrypt_context_t */*!\hlblue{ctx}!*/) {
  int /*!\hlblue{fd}!*/ = open(/*!\hlblue{"secret\_key"}!*/, /*!\label{line:fd-sign}!*/ /*!\hfill\action{PATH-Auth + FD-Sign}!*/ 
                O_RDONLY);
  /*!\hlblue{ctx->secret\_key}!*/    /*!\label{line:ptr-sign}!*/  /*!\hfill\action{PTR-Sign}!*/
    = capac_malloc(KEY_SIZE);
  read(/*!\hlblue{fd}!*/, /*!\hlblue{ctx->secret\_key}!*/, KEY_SIZE);   /*!\hfill\action{FD-Auth}!*/ 
}
DOM_PRIV_STACK
void encrypt( DOM_PRIV encrypt_context_t /*!\hlblue{ctx}!*/, 
        char **/*!\hlgray{plaintext}!*/, char **/*!\hlgray{ciphertext}!*/) {
  for(int i = 0; i < size; i++)
    /*!\hlgray{*ciphertext}[i]!*/ =  /*!\label{line:ptr-sign}!*/  /*!\hfill\actionambient{PTR-Auth}!*/
        /*!\hlblue{ctx->secret\_key}!*/ ^  /*!\label{line:ptr-sign}!*/  /*!\hfill\action{PTR-Auth}!*/
        /*!\hlgray{*plaintext}[i]!*/; /*!\label{line:ptr-sign}!*/  /*!\hfill\actionambient{PTR-Auth}!*/
}
/*!
\begin{flushleft}
{\sffamily \footnotesize
\noindent\hlblue{\ \ \ \ \ \ \ \ } : Domain-private objects
\\
\hlgray{\ \ \ \ \ \ \ \ } : Ambient objects
\\
\action{Action}/\actionambient{Action} : \thename's actions on domain-priv./ambient ref.
\\
\secreq{Component} : \thename's component enforcing action 
}
\end{flushleft}
!*/
\end{lstlisting}

\end{minipage}
\hfill
\begin{minipage}[t]{.47\textwidth}
% \begin{minipage}[t]{.40\textwidth}
% \begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{ssblue!10},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,framexrightmargin=10pt,belowskip=1pt ,name=entrylib]
% entry_token_t token = pacga(target_dom);
% domain_switch_ioctl(token);
% dom_curr = target_dom;
% \end{lstlisting}
% \end{minipage} 
% \hspace{11pt}
% \begin{minipage}[t]{.5\textwidth}
% \begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{ssblue!11},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt, name=entrykernel]
% dom_id_t target_dom = authenticate_entry(token);
% switch_domain_key(target_dom);
% \end{lstlisting}
% \end{minipage} 
 
\begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{ssblue!10},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt, name=memalloc]
int tag = dom_auth();
if (tag == FAILED) return NULL;
// Allocates tagged memory and return tagged PTR
return alloc_priv_mem(size, tag);
\end{lstlisting}

% \begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{ssblue!10},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt, name=pathauth]
% authenticate_path("secret_key.txt", kernel_secret);
% int raw_fd = sys_open("secret_key.txt", O_RDONLY);
% return sign_fd(raw_fd, kernel_secret);
% \end{lstlisting}
\begin{minipage}[t]{.40\textwidth}

\end{minipage}
\hspace{2.7cm}
\begin{minipage}[t]{.66\textwidth}
% \begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{ssblue!10},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,framexrightmargin=10pt,belowskip=1pt ,name=entrylib]
% entry_token_t token = pacga(target_dom);
% domain_switch_ioctl(token);
% dom_curr = target_dom;
% \end{lstlisting}
% \end{minipage} 
% \hspace{11pt}
% \begin{minipage}[t]{.5\textwidth}
% \begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{ssblue!11},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt, name=entrykernel]
% dom_id_t target_dom = authenticate_entry(token);
% switch_domain_key(target_dom);
% \end{lstlisting}
% \end{minipage} 

% Hack to allocate  space for figure
\begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{ssblue!10},frame=shadowbox,framesep=3pt,framexleftmargin=1pt,belowskip=-5pt, name=refmon,framextopmargin=3cm]
\end{lstlisting}
\end{minipage}

\usetikzlibrary{shapes.geometric, arrows}

\tikzstyle{process} = [rectangle, minimum width=.5cm, minimum height=.2cm, anchor=west ,font=\fontsize{8}{8}\ttfamily, draw=black,fill=white, inner sep=.05cm]
\tikzstyle{decision} = [diamond, minimum width=.2cm,aspect=1.5, minimum height=.2cm, text centered,font=\fontsize{8}{8}\ttfamily, draw=black,fill=white, inner sep=.1cm]
\tikzstyle{arrow} = [->,>=latex]
\tikzstyle{funccall} = [text centered,font=\fontsize{8}{8}\ttfamily,anchor=west]

\begin{tikzpicture}[
  remember picture,
  overlay,
]

% Anchor point
\draw (pic cs:line-refmon-1-start) node (pathaut) [decision,yshift=1.7cm,xshift=4.7cm] {AUT};

% Nodes that are on the same line
\node (fdpac) [process, right of=pathaut, xshift=1.6cm, inner sep=.2cm] {PAC};
\node (fdaut) [decision, below of=pathaut, yshift=-.1cm] {AUT};


\node (fdautfail) [right of=fdaut, xshift=.3cm] {};


% Nodes on the line above
\node (sysopen) [process,left of=pathaut, yshift=0cm, xshift = -2.3cm, text width=2.4cm] { int fd =    open(\\\hlblue{"secret\_key"},...)};
\node (sysread) [process,left of=fdaut, yshift=0cm, xshift=-2.3cm, text width=2.4cm] {read(\hlblue{fd},...)};



% Nodes on the line below
% \node (pathautfail) [below of=pathaut, yshift=-.2cm] {};
\node (dosysopen) [process, above of=fdpac] {do\_sys\_open(...)};
\node (dosysread) [process, right of=fdaut, xshift=1.8cm] {do\_sys\_read(...)};

\node (inode) [process, above of=pathaut, inner sep=.07cm] {struct inode};
\draw [arrow] (inode) -- node[funccall,anchor=east]{f\_security}(pathaut) ;
% True arrows
\draw [arrow] (pathaut) to[out=0,in=180]  node[funccall,anchor=north,right]{Success} (dosysopen) ;
\draw [arrow] (fdaut) -- node[funccall,anchor=south]{Success}(dosysread);

% % false arrows
% \draw [arrow] (fdaut) -- node[funccall,anchor=south]{F}(fdautfail);
% \draw [arrow] (pathaut) -- node[funccall,anchor=west]{F}(pathautfail) ;

\draw [arrow] (fdpac) to[out=south,in=south,looseness=.12] node[funccall,xshift=2cm,yshift=.1cm]{\hlblue{fd}}(sysopen);
\draw [arrow] (sysread) -- (fdaut);
\draw [arrow] (sysopen) -- (pathaut);
\draw [arrow] (dosysopen) -- node[funccall,anchor=west]{fd} (fdpac);

\draw [arrow] ([yshift=.8ex,xshift=-1ex] pic cs:line-codeexample-12-end) to[out=0,in=180] (sysopen);
\draw [arrow] ([yshift=.8ex,xshift=-1ex] pic cs:line-codeexample-16-end) to[out=0,in=180] (sysread);
% Label

% divider 
% \draw ([yshift=1.9cm,xshift=.2cm]pic cs:line-refmon-1-start) -- ([yshift=1.9cm,xshift=.42cm+\textwidth]pic cs:line-refmon-1-end);
\draw (pic cs:line-refmon-1-start) node[yshift=3.2cm,xshift=4.0cm]{\secreq{Reference monitor}};
% % \draw (pic cs:line-refmon-1-start) node[yshift=2.4cm,xshift=2.8cm, above]{\action{PATH-Auth}};
\node[left of=pathaut,below]{\scriptsize\action{PATH-Auth}};
\node[left of=fdaut,below]{\scriptsize\action{FD-Auth}};
\node[right of=fdpac,xshift=-.05cm]{\scriptsize\action{FD-Sign}};
% % \draw (pic cs:line-refmon-1-start) node[yshift=2.4cm,xshift=5.2cm, above]{\action{FD-Sign}};
% \node[right of=fdpac,above,xshift=-.1cm]{\action{FD-Sign}};
% \node[left of=fdaut,below,xshift=.1cm]{\action{FD-auth}};
% \draw (pic cs:line-refmon-1-start) node[]{\action{FD-Auth}};


\end{tikzpicture}


% \includesvg[width=\textwidth]{images/ref-mon-actions.svg}
% \includegraphics[width=1.055\textwidth]{images/ref-mon-actions.pdf}

% \begin{lstlisting}[style=sslab-mini-c,language={C},keepspaces,numbers=none,backgroundcolor=\color{ssblue!10},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt, name=fdauth]
% int raw_fd = authenticate_fd(fd, kernel_secret);
% return sys_read(raw_fd);
% \end{lstlisting}


\begin{lstlisting}[style=sslab-mini-c,language={[ARM]Assembler},keepspaces,numbers=none,backgroundcolor=\color{ssblue!10},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt,name=domptrsign]
/*!\textbf{pacdz}!*//*!\underline{\textbf{b}}!*/  ptr         //    
str	    ptr, [mem]  // Store PTR into memory
\end{lstlisting}
\begin{lstlisting}[style=sslab-mini-c,language={[ARM]Assembler},keepspaces,numbers=none,backgroundcolor=\color{ssblue!10},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt,name=domptrauth]
ldr     ptr, [mem]  // Load domain-priv. PTR from memory
/*!\textbf{autdz}!*//*!\underline{\textbf{b}}!*/  ptr         // 
\end{lstlisting}
\begin{lstlisting}[style=sslab-mini-c,language={[ARM]Assembler},keepspaces,numbers=none,backgroundcolor=\color{lgray!40},frame=shadowbox,framesep=3pt,framextopmargin=3pt,framexleftmargin=1pt,belowskip=1pt, name=ambptrauth]
ldr     ptr, [mem]  // Load ambient PTR from memory
/*!\textbf{autdz}!*//*!\underline{\textbf{a}}!*/  ptr         //
\end{lstlisting}
\end{minipage}
\begin{tikzpicture}[
  remember picture,
  overlay,
  annotation/.style={
    inner sep=0pt,
    outer sep=0pt,
    outer xsep=1mm,
    text width=5cm
  },
%   >={Stealth[inset=0pt, angle=45:7pt]}
]
\newcommand{\codeboxyshift}{1.8ex}
\newcommand{\codeboxxshift}{2.5cm}
\newcommand{\componentxshift}{6cm}


\draw (pic cs:line-entrylib-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=\codeboxxshift]{\action{capac\_enter}};
\draw (pic cs:line-entrylib-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=4.7cm]{\secreq{\libcapac}};


\draw (pic cs:line-entrykernel-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=\codeboxxshift]{\action{capac\_enter}};
\draw (pic cs:line-entrykernel-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=4.7cm]{\secreq{Reference Monitor}};

\draw (pic cs:line-pathauth-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=\codeboxxshift]{\action{PATH-Auth+FD-Sign}};
\draw (pic cs:line-pathauth-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=5.8cm]{\secreq{Reference Monitor}};


\draw (pic cs:line-fdauth-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=\codeboxxshift]{\action{FD-Auth}};
\draw (pic cs:line-fdauth-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=5.8cm]{\secreq{Reference Monitor}};



% \draw (pic cs:line-domptrsign-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=\codeboxxshift]{\action{PTR-Sign}};

% \draw (pic cs:line-domptrauth-1-start) node[annotation, ,xshift=\codeboxxshift]{\action{PTR-Auth}};

% \draw (pic cs:line-ambptrauth-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=\codeboxxshift]{\actionambient{PTR-Auth}};
\draw (pic cs:line-domptrsign-1-end) node[annotation, right,yshift=0.1cm,xshift=-0.1cm]{\action{PTR-Sign}};
\draw (pic cs:line-domptrauth-2-end) node[annotation, right,yshift=0.05cm,xshift=-0.1cm]{\action{PTR-Auth}};
\draw (pic cs:line-ambptrauth-2-end) node[annotation, right,yshift=0.05cm,xshift=-0.1cm]{\actionambient{PTR-Auth}};

\draw (pic cs:line-memalloc-1-start) node[annotation, above, yshift=0cm,xshift=9cm]{\action{capac\_malloc()}};



% Headers
\draw (pic cs:line-memalloc-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=2.3cm]{\secreq{\libcapac}};

\draw (pic cs:line-domptrsign-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=2.3cm]{\secreq{Instrumentation Framework}};

\draw (pic cs:line-domptrauth-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=2.3cm]{\secreq{Instrumentation Framework}};

\draw (pic cs:line-ambptrauth-1-start) node[annotation, above, yshift=\codeboxyshift,xshift=2.3cm]{\secreq{Instrumentation Framework}};
\end{tikzpicture}

\newcommand{\titleyshift}{3.3ex}
\newcommand{\titlexshift}{.7ex}
\begin{tikzpicture}[remember picture,overlay,>=Latex]
% \draw[->] (pic cs:line-codeexample-5-end)  to[out=0,in=170] ([yshift=\titleyshift,xshift=\titlexshift] pic cs:line-entrylib-1-start);
% \draw[->] ([yshift=.8ex,xshift=-1ex] pic cs:line-codeexample-12-end) to[out=0,in=170] ([yshift=\titleyshift,xshift=\titlexshift] pic cs:line-pathauth-1-start);
% \draw[->] ([yshift=.8ex,xshift=-1ex] pic cs:line-codeexample-16-end) to[out=0,in=170] ([yshift=\titleyshift,xshift=\titlexshift] pic cs:line-fdauth-1-start);


% \draw[->] ([yshift=.8ex,xshift=-1ex] pic cs:line-codeexample-14-end) to[out=0,in=170] ([yshift=\titleyshift,xshift=\titlexshift] pic cs:line-domptrsign-1-start);


\draw[->] ([yshift=.8ex,xshift=-1ex] pic cs:line-codeexample-14-end) to[out=0,in=180] ([xshift=-.2cm] pic cs:line-domptrsign-1-start);
\draw[->] ([yshift=.8ex,xshift=-1ex] pic cs:line-codeexample-23-end) to[out=0,in=180] ([xshift=-.2cm] pic cs:line-domptrauth-1-start);
\draw[->] ([yshift=.8ex,xshift=-1ex] pic cs:line-codeexample-24-end) to[out=0,in=180] ([xshift=-.2cm] pic cs:line-ambptrauth-1-start);
% \draw[->] ([yshift=.8ex,xshift=-1ex] pic cs:line-codeexample-25-end) to[out=0,in=170] ([yshift=\titleyshift,xshift=\titlexshift] pic cs:line-ambptrauth-1-start);
% \draw[->] (listings-13) -- (listings-11);
% \draw[->] (listings-11) -- (listings-6);
% \draw[->] (listings-6) to[out=-45,in=-135] (listings-7);
% \draw[->] (listings-7) to[out=-45,in=-135] (listings-9);
\end{tikzpicture}


\caption{Example of \thename's domain-private objects, \thename's actions and components that enforce their isolation.}
\label{fig:code-example}
\end{figure*}

==> sections/__old-intro.tex <==
\section{Introduction}
\label{sec:intro}
% \IEEEPARstart{M}{odern}


Modern software is often large and complex. As a result, it suffers from bugs, some of which are security vulnerabilities that concede program control to adversaries or leak sensitive program resources (e.g., cryptographic keys). However, completely eradicating bugs is a rather unrealistic goal. Researchers and industry have resorted to separating a single program into multiple compartments~\cite{aces,privman,privtrans,wedge,hakc,muscope}, each ideally performing a specific task (\emph{separation of privilege}) and is granted only the essential privileges (\emph{least privilege}).

Given the high overheads incurred by dividing a program into multiple processes, many works have proposed \gls{ipi}~\cite{lotrx86,shreds,seimi,erim,hodor,jenny,cerberus,donky} to provide low-overhead isolation of in-process \emph{domains}. Many of such designs utilize either repurposing of existing hardware features~\cite{lotrx86,shreds} or adaptation of newly introduced hardware features~\cite{hodor,erim,jenny,cerberus} such as Intel's \gls{pku}~\cite{intel-manual} that makes use of memory protection automatically enforced by the \gls{mmu}. 
\st{Besides, the necessity and design space of efficient process reference monitors for {\gls{ipi}} schemes have been discussed in many previous works~{\cite{pku-pitfall,jenny,cerberus,monguard}}. Researchers have shown that the {\gls{ipi}}-unaware kernel may inadvertently serve as a confused deputy who allows the adversary to undermine the security of the protected domains~{\cite{pku-pitfall,jenny}}. As such, many works introduce reference monitor designs for {\gls{ipi}} to mediate the insecure interfaces between the untrusted domains and the kernel through system calls filtering~{\cite{jenny,cerberus,monguard}}. To this end, our work presents a reference monitor design that enables the simple and efficient authentication of file object references through hardware cryptographic primitives.}


However, many of the works on \gls{ipi} leverage \gls{pku}~\cite{erim,hodor,jenny,cerberus} which is only available on x86. \gls{ipi} on ARM was previously explored~\cite{shreds} using AArch32's \emph{domains} memory protection feature that had an uncanny resemblance to \gls{pku}. However, the domains feature has now been deprecated in AArch64. On embedded ARM processors such as the Cortex-M, \gls{ipi} is only explored on embedded and bare-metal systems to provide a rudimentary separation of components with limited hardware supports~\cite{epoxy,minion,mbedos,aces}. Proposals for \gls{ipi} designs on the modern ARM architectures are lacking to the best of our knowledge. 

The ARM processor architecture's recent iterations introduced new hardware-assisted software security features. \Gls{pa}~\cite{arm-arch,armv8-m}, is a hardware feature in ARMv8.3 \st{and the low-powered ARMv8-M that }implements the principles from CCFI~\cite{ccfi} and CPI~\cite{cpi}. \Gls{pa} introduced the kernel-managed key registers, as well as dedicated instructions for signing and authenticating pointers. Software defenses that utilize \gls{pa} prevent the use of corrupted pointers by signing the pointers with \glspl{pac} before storing them in memory. The signed pointers are then authenticated when loaded from memory into a register or immediately before use. \gls{mte} is another hardware feature included in the ARMv8.5-A architecture to enable tagging of pointers and the \emph{pointee} 16-byte memory blocks. \gls{mte}-enabled processors throw an exception when it detects a tag mismatch between the pointer and the memory location. Notably, \gls{pa} and \gls{mte} can be enabled simultaneously such that the pointers are tagged \emph{and} signed.

Our work explores a new \gls{ipi} model that revolves around the capability-based security principle~\cite{obj-cap,eros}, a design choice that fully exploits the new hardware extensions in modern ARM architecture. In capability-based systems, the proof of access rights travels with the references to the objects, providing fine-grained and in-place access control to programmers. As such, access control decisions in capability systems are made by authenticating and verifying the integrity of the non-forgeable references to the objects. Capability-based access control has been discussed in the context of memory safety~\cite{cheri,cheri-risc,cheriabi,lowfat-pointer,new-lowfat-pointer}. The CHERI architecture~\cite{cheri,cheri-risc,cheriabi} applies memory capabilities to pointers, although it requires a customized processor architecture. On the other hand, our work proposes using the new ARM hardware features. Another difference is that our work is more comprehensive in that it applies capability on \emph{both} pointers and file object references. Capsicum~\cite{capsicum} explored a set of kernel changes to retrofit POSIX access control with capability principles. However, it assumes process-level program compartmentalization while our work seeks to provide capability-based access control for intra-process entities.


In this paper, we propose \thename, a novel capability-based \gls{ipi} model based on the observation that the two hardware features, \gls{pa} and \gls{mte}, are, in fact, object capability. Our design undertakes unique challenges as it embarks on a vastly different approach compared to the existing \gls{ipi} methods that adapt \gls{mmu}-based isolation. \thename creates in-process \emph{domains}, subprogram components that are given exclusive access to sensitive process resources. Each domain is identified and authenticated by their \emph{domain authentication keys}, or domain keys. \thename encapsulates all files and memory references with authentication codes generated using the domain keys of the owner. Hence, the references can only be successfully authenticated while the context executes within the owner domain. \thename also rigorously assesses and addresses the security requirements for the capability references, namely the \emph{non-forgeability} and \emph{non-reusability} requirements. 

\thename implements a reference monitor and an instrumentation framework to achieve complete mediation, which is an imperative premise for capability-based access control. The reference monitor is a minimal kernel module that interposes system calls to enforce fast cryptographical authentication through \gls{pa} instructions. Such fast authentication is possible because the references themselves carry sufficient information for access control decisions in a non-forgeable way, allowing reference monitor design to be simplified. Moreover, \thename shows that domain memory isolation can be established through its tagged and cryptographically-authenticated pointers, whose creation and authentication are accelerated by \gls{pa} and \gls{mte}. Based on this, \thename introduces an instrumentation framework and a supporting library to guarantee that all accesses to memory are authenticated and tag-checked. \thename's use of hardware primitives allows it to achieve a relatively low performance overhead.




In summary, we outline the contributions of this work as the following:


\begin{itemize}[leftmargin=1.0em]
\setlength\itemsep{-0.1em}
\item We introduce a novel intra-process isolation design that implements hardware-accelerated capability on ARM.
\item We assess and address the unique security challenges of capability-based intra-process isolation that requires complete mediation on reference uses and prevention of forging and reusing of the references.
\item We show life cycle protection of sensitive domain resources by protecting both file and memory references.
\item We evaluate our implementation through a real-world application and report low overhead on the new \gls{ipi} approach.
\item We make our implementation publicly available\footnote{A link to the repository will be available in the final version} in the hopes of contributing to future directions in capability-based \gls{ipi}.
\end{itemize}

\iffalse
Modern software is often large and complex.
As a result, it suffers from bugs, some of which are security vulnerabilities that concede program control to adversaries or leak sensitive program resources (\eg, cryptographic keys).
However, completely eradicating bugs is a rather unrealistic goal.
Researchers and industry have resorted to separating a single program into multiple compartments~\cite{aces,privman,privtrans,wedge,hakc,muscope}, each ideally performing a specific task (\emph{separation of privilege}) and is given only the essential privileges (\emph{least privilege}).

Given the high overheads incurred by dividing a program into multiple processes, many works have proposed \gls{ipi}~\cite{lotrx86,shreds,seimi,erim,hodor,jenny,cerberus,donky} to provide low-overhead isolation of in-process security domains.
% Two prominent approaches to achieve \gls{ipi} are \gls{sfi}, which employs the compiler to transform programs into sandboxed modules~\cite{nacl,nacl-ext,rlbox,webassembly} and 
Many of such works either re-purposes existing hardware features~\cite{lotrx86,shreds,seimi} or adapts of newly introduced hardware features~\cite{pkrusafe,hodor,erim,jenny,cerberus} such as Intel's \gls{pku} and ~\cite{intel-manual}.
Recent works have demonstrated that \gls{pku}-based isolation achieves significantly better performance compared to per-process isolation and \gls{sfi}~\cite{nacl,nacl-ext,rlbox,webassembly} thanks to low-cost context switches~\cite{erim,hodor}.
Hardware-assisted \gls{ipi} on ARM was previously explored~\cite{shreds} using \emph{domains} memory protection feature that had an uncanny resemblance to \gls{pku}.
However, the domains feature has now been supported in AArch64.
Proposals for \gls{ipi} designs on the modern ARM architectures are lacking to the best of our knowledge.



% On embedded ARM processors such as the Cortex-M, \gls{ipi} is only explored on embedded and bare-metal systems to provide a rudimentary separation of components with limited hardware supports~\cite{epoxy,minion,mbedos,aces}.

The ARM processor architecture's recent iterations introduced new hardware-assisted software security features.
\Gls{pa}~\cite{arm-arch,armv8-m}, is a hardware feature in ARMv8.3 that implements the principles from CCFI~\cite{ccfi} and CPI~\cite{cpi} to protects pointers from corruption.
\gls{mte} is another hardware feature included in the ARMv8.5-A architecture to enable tagging of pointers and the \emph{pointee} 16-byte memory blocks.
\gls{mte}-enabled processors to throw an exception when it detects a tag mismatch between the pointer and the memory location.
Our work introduces an \gls{ipi} model that takes advantage of both \gls{pa} and \gls{mte} by coherently combining their security guarantees.


In this paper, we propose \thename, a novel capability-based \gls{ipi} model that is based on the observation that two hardware features, \gls{pa} and \gls{mte}, have characteristics of of \emph{capability-based access control} (or simply \emph{capability}).
Previous works in the realms of OS and memory safety have discussed capability as the ideal scheme for achieving the \emph{least privilege} compartments and eliminating \emph{ambient authority} of software systems~\cite{cheri,capsicum,eros}.
As a capability system, the access control decisions in \thename are made by authenticating and verifying the integrity of the non-forgeable references to the objects, whose construction is accelerated by \gls{pa} and \gls{mte}.

% In capability-based systems, the proof of access rights travels with the references to the objects, providing programmers fine-grained and in-place access control.
% As such, access control decisions in capability systems are made by authenticating and verifying the integrity of the non-forgeable references to the objects.

Our design undertakes unique challenges as it embarks on a vastly different approach compared to the existing \gls{ipi} methods that adapt \gls{mmu}-based isolation (\eg, Intel PKU~\cite{erim,hodor,libmpk}).
\thename creates in-process \emph{domains}, subprogram components that are given exclusive access to sensitive process resources.
Each domain is identified and authenticated by their \emph{domain authentication keys} (or domain key), which is a \gls{pa} cryptographic key that \thename reserved authenticating resources.
\thename encapsulates all files and memory references with authentication codes generated using the domain keys of the owner.
Hence, the references can only be successfully authenticated while the context executes within the owner domain.
\thename also rigorously assesses and addresses the security requirements for the capability references, namely \emph{non-forgeability} and \emph{non-reusability}.

\thename implements a reference monitor and an instrumentation framework to achieve complete mediation, which is an imperative premise for capability-based access control.
The reference monitor is a minimal kernel module that interposes system calls and enforces cryptographical authentication on the resource accesses (\eg, sockets and files) with \gls{pa} instructions.
\thename's resource authentication is both \emph{fast} and \emph{simple} because the references (\thename-signed file descriptors) themselves carry sufficient information for access control decisions in a non-forgeable way.
\thename establishes domain memory isolation through its tagged and cryptographically-authenticated pointers, whose creation and authentication are accelerated by \gls{pa} and \gls{mte}.
\thename introduces an instrumentation framework that inserts inline \gls{pa}-based security checks to mediate pointer usages and a supporting runtime library that facilitates the secure creation of domain-private memory.

\fi

==> sections/__old_design.tex <==



\iffalse
\thename's instrumentation framework enforces domain memory isolation through tagging domain-private memory regions and completely mediating memory access through pointers that are made non-reusable (\srreuse) and non-forgeable (\srforge) token of memory access rights.  
% It implements a \emph{domain-aware} pointer authentication scheme in which all pointer store and load sites to ambient and domain-private memory regions are distinguished, then signed and authenticated with different keys (\key{DA} vs. \key{DB}).

% \autoref{fig:asm} shows snippets of a \thename-instrumented functions. A complete instrumented function is displayed in \cref{sec:asm}.




% \thename instrumentation adapts \emph{on-load} pointer authentication scheme~\cite{pac-it-up}. 
% More specifically, \thename instruments the program to sign pointers as before they are stored in memory and authenticate pointers as they are loaded from memory into registers, as shown by the following code example.

% \vspace{-1em}
% \noindent%
% \begin{minipage}[t]{.45\columnwidth}
% \begin{lstlisting}[style=sslab-mini-c,frame=none,language={[ARM]Assembler},keepspaces,numbers=none]
% // ptr: domain-priv. ptr.
% /*!\textbf{pacdz}!*//*!\underline{\textbf{b}}!*/  ptr  /*!\hfill\action{PTR-Sign}!*/
% str	    ptr, [mem]  
% ...
% ldr     ptr, [mem] 
% /*!\textbf{autdz}!*//*!\underline{\textbf{b}}!*/  ptr /*!\hfill\action{PTR-Auth}!*/
% \end{lstlisting}
% \end{minipage}%
% \begin{minipage}[t]{.45\columnwidth}
% \begin{lstlisting}[style=sslab-mini-c,frame=none,language={[ARM]Assembler},keepspaces,numbers=none]
% // ptr: ambient ptr.
% /*!\textbf{pacdz}!*//*!\underline{\textbf{a}}!*/  ptr /*!\hfill\actionambient{PTR-Sign}!*/
% str	    ptr, [mem]  
% ...
% ldr     ptr, [mem] 
% /*!\textbf{autdz}!*//*!\underline{\textbf{a}}!*/  ptr /*!\hfill\actionambient{PTR-Auth}!*/ 
% \end{lstlisting}
% \end{minipage}

%Compared to an \emph{on-use} authentication scheme that authenticates every pointer dereferences, on-load authentication provides a reasonable trade-off between performance and security~\cite{pac-it-up}. In brief, the following instrumentation is inserted for load/store instructions that access ambient/domain-private pointers:



% \thename establishes domain memory isolation through two techniques.
% First, \thename adapts \gls{mte} to tag domain-private memory regions with \tagnum{Dom} of the owner domain, which ensures that only the same-tag pointers can access such tagged memory.
% Second, \thename completely mediates \ptr accesses through whole-program instrumentation for \emph{domain-aware authentication} that \emph{selectively} authenticates domain-private {\ptr}s with \key{DB}, and uses \key{DA} otherwise.
% As shown in \autoref{fig:ref}, a \thename's \ptr reference is both \gls{mte}-tagged and \gls{pa}-signed.



\hdr{Domain-private memory tagging}
\iffalse
\thename establishes domain-private memory regions through the use of \gls{mte} memory tagging. Each domain's private memory is tagged with the domain's integer domain ID (\tagnum{Dom}), and only pointers that are tagged with the same ID can be used to access it. The adaption of \gls{mte} is imperative as \gls{pa} alone is incapable of ensuring memory isolation; an adversary can authenticate a pointer and then perform an out-of-bounds memory access (e.g., \texttt{gets(autda(ptr))}). Recall that the ambient domain is assigned a domain ID of \emph{0}. This intentional choice renders all untagged memory pointers to be ambient memory references while only the deliberately tagged pointers become references to domain-private memory.

\thename has two types of tagged memory generation sites. First, \texttt{capac\_malloc()} (explained in \cref{sec:design:libcapac}) facilitates runtime allocation and just-in-time tagging of heap memory. Upon invocation, \texttt{capac\_malloc(size)} first performs \gls{dst}-based domain authentication so that it can determine the tag number of the currently executing domain as we explained in \cref{sec:design:switch-auth}. Afterward, \texttt{capac\_malloc()} allocates memory from its memory pool, tags the memory with the domain ID, then finally returns a pointer also tagged with the domain ID. Note that the returned pointer is not signTed as it is delivered in the return value register, adhering to \thename instrumentation's on-store sign and on-load authentication policy.

Second, \thename provides private \emph{stack} memory to domains through in-place tagging and untagging of the stack objects with the current domain ID (i.e., no explicit stack switching). The \texttt{CAPAC\_STACK} directive shown in line 8 of \autoref{fig:code-example} notifies the instrumentation framework to instrument the function prologue and epilogue to prepare a domain-private stack before the function execution proceeds and also to untag and zero out the tag before return respectively. The instrumented prologue authenticates and obtains the currently executing domain's ID by consulting \gls{dst} (shown in \autoref{fig:asm-prologue}). Then, it tags the function's stack frame using the retrieved ID as a \gls{mte} tag as shown in \autoref{fig:asm-stack-tagging}. The epilogue (\autoref{fig:asm-epilogue}) returns the stack frame back to the ambient domain by zeroing out the stack contents and setting the tag on the memory region back to 0. The instrumentation uses \texttt{stzg} instruction introduced in \gls{mte} that performs such operation efficiently in the hardware.

\hj{There are two sources of domain-private memory in \thename: tagged heap memory returned by \texttt{capac\_malloc()} (explained in \cref{sec:design:libcapac}) and tagged function stack frame allocation activated by the \texttt{DOM\_PRIV\_FUNC} function attribute.} 
%We implement the stack tagging instrumentation based on the built-in stack tagging LLVM instrumentation on AArch64~\cite{llvm-stack-tagging}.
The instrumentation enables domain-private stack memory through in-function tagging and untagging of the stack objects with the current domain ID, and this allows us to avoid complete stack switching during domain switches.
The instrumented function's prologue consults the \texttt{libcapac}'s \gls{dst} to authenticate the current domain and obtain the \tagnum{Dom} of the current domain.
From this point on, the \tagnum{Dom} is to tag every stack allocation (LLVM's \texttt{alloca}) and also the resulting pointer.
In the instrumented function's epilogue, the stack is zeroed out then untagged (\tagnum{Ambient} = 0) before returning. The instrumentation uses \texttt{stzg} instruction introduced in \gls{mte} that performs this particular operation efficiently in the hardware. 

% \thename instrumentation framework insert memory tagging instructions to the prologue and epilogue of a function annotated with \texttt{DOM\_PRIV\_FUNC} (\cref{sec:design:instrumentation}).
\fi 
% USENIX
\thename establishes domain-private memory regions through the use of \gls{mte} memory tagging. Each domain's private memory is tagged with the domain's integer domain ID (\tagnum{Dom}), and only pointers that are tagged with the same ID can be used to access it. The adaption of \gls{mte} is imperative as \gls{pa} alone is incapable of ensuring memory isolation; an adversary can authenticate a pointer and then perform an out-of-bounds memory access (e.g., \texttt{gets(autda(ptr))}). Recall that the ambient domain is assigned a domain ID of \emph{0}. This intentional choice renders all untagged memory pointers to be ambient memory references while only the deliberately tagged pointers become references to domain-private memory.

\thename has two sources of tagged memory generation. First, \texttt{capac\_malloc()} facilitates runtime allocation and just-in-time tagging of heap memory. Upon invocation, \texttt{capac\_malloc(size)} first performs \gls{dst}-based domain authentication so that it can determine the tag number of the currently executing domain as we explained in \cref{sec:design:switch-auth}. Afterward, \texttt{capac\_malloc()} allocates memory from its memory pool, tags the memory with the domain ID, then finally returns a pointer also tagged with the domain ID. Note that the returned pointer is not signed as it is delivered in the return value register, adhering to \thename instrumentation's on-store sign and on-load authentication policy.

Second, \thename provides private \emph{stack} memory to domains through in-place tagging and untagging of the stack objects with the current domain ID (i.e., no explicit stack switching). The \texttt{DOM\_PRIV\_FUNC} directive notifies the instrumentation framework to instrument the function prologue and epilogue to prepare a domain-private stack before the function execution proceeds and also to untag and zero out the tag before return, respectively. The instrumented prologue authenticates and obtains the currently executing domain's ID (\cref{sec:design:libcapac}. Then, it tags the function's stack frame using the retrieved ID as a \gls{mte} tag. The epilogue returns the stack frame back to the ambient domain by zeroing out the stack contents and setting the tag on the memory region back to 0. 
The instrumentation uses \texttt{stzg} instruction introduced with \gls{mte} that performs this particular operation efficiently in the hardware. 


\hdr{Domain-aware pointer authentication}
\thename instrumentation framework must mediate the creation of authenticated pointers to the tagged domain-private memory and timely authentication of the pointers being loaded. That is, such domain-private pointers must be successfully authenticated only within its owner domain execution context. For this objective, the instrumentation must identify all pointers that point to domain-private memory and enforce the DPI scheme to selectively sign (\action{PTR-Sign}) and authenticate (\action{TPTR-Auth}) the pointers using the domain authentication key, \key{DB}.

\fi

\iffalse
\SetKw{KwInput}{Input:}
\SetKw{KwOutput}{Output:}
\begin{algorithm}[t]
\footnotesize
% $P\gets\{\emptyset\}$\;
% \tcc{Pointers that may contain}
% $D\gets\{\emptyset\}$\;
\KwInput{$A$ = Set of annotated \texttt{alloca} instructions}\;
\KwOutput{$D$ = Set of sensitive IR variables}\;
$Worklist \gets \{A\}$\;
$D \gets \{\emptyset\}$\;
\For{Instruction $I$ in $Worklist$}{
    \If{isAddressingInst($I$) $\cup$ isPointer($I$.pointeeType)}{
        $D \gets \{ D \cup I \}$\;
    }
    \For {Instruction $U$ that uses $I$}{
        \If{isStoreInst($U$)}{
            \If{$I == U.valueOperand$}
            {
                $Worklist \gets \{Worklist \cup U.pointerOperand\}$\;
            }
            \Else{
                $Worklist \gets \{Worklist \cup U.valueOperand\}$\;
            }
        }
        \ElseIf{isLoadInst($U$)}{
            $Worklist \gets \{Worklist \cup U.pointerOperand\}$\;
        }
        \Else{
            $Worklist \gets \{Worklist \cup U\}$\;
        }
    }
}
\caption{Domain-private \ptr taint tracking}
\label{algo:taint-tracking}
\end{algorithm}
\fi

\iffalse
\autoref{fig:overview} illustrates an overview of \thename capability model, which incorporates hardware security features of the recent and upcoming ARM architecture, whose principles and directions exhibit capability characteristics.
At a high level, \thename identifies \emph{domains} as subgraphs of program execution that interact with in-process objects, \eg, files and memory objects.
\thename authenticates domains through per-domain \gls{pa} keys securely maintained inside the kernel.
We refer to \emph{\thename domains} as identified domains that are encapsulated between the domain entry (\texttt{capac\_enter(DOM\_ID)}) and exit (\texttt{capac\_exit()}), and the remaining of the program as the \emph{ambient domain}.

The primary objective of \thename is to guarantee that the \thename domains have exclusive access to their program objects.
It transforms the in-process objects (e.g., file descriptors and memory pointers) into domain-exclusive capability tokens, or \thename references, by cryptographically binding them with \glspl{pac} using the per-domain \gls{pa} key.
\thename ensures all of its references are authenticated before being used, which is achieved through its \emph{complete mediation} that scheme we will explain in \cref{sec:implementation}.
\fi
% \added{
% \thename introduces a flavor of capability that is \emph{coherent} between different types of resources. 
% Existing works introduced capability-based security that protects different types of resources, file descriptors \cite{capsicum}, or memory pointers \cite{cheri,cheriabi}.
% On the other hand, \thename provides an access control scheme that covers the \emph{life-cycle} of sensitive resources, from the file system reference (path string) to the object's in-memory representation.
% }

% \added{
% \thename's uses of \gls{pa} hardware primitive greatly simplify its reference authentication design.
% With a single check on the reference with an \texttt{autxx} instruction, \thename can authenticate if (1) The reference belongs to the currently executing domain and (2) The reference has not been tampered with. 
% Cryptographically-secured object references in \thename are coherently built into the program through a \thename library, in-kernel monitor, and compiler instrumentation. Managing the access control on sensitive system objects in \thename is achieved through in-place annotations and is enforced automatically by \thename's facilities.
% }




% In \thename, the access control decisions on the references are made using a simple \gls{pa}-based cryptographic authentication. 
% This elegant design allows for efficient hardware-accelerated enforcement, and also allows for.
% instead of relying on complex logic for .


% It utilizes a unified mechanism for access control
% % , instead of relying on separate logic for resource authentication.
% % For instance, 
% Not only coherent, \thename capability is also efficient due to pa and mte
% \added{
% \added{
% Moreover, \thename's capability scheme is \emph{lightweight}. 
% \thename is able to guaratee non-usability of references across domains or resources without a complex modifier management. 
% \thename's  does not require additional kernel data structures, such.  
% \thename introduces a novel \emph{hardware-enhanced capability model} that incorporates    
% }
% Unlike previous models that requires separate logic
% }




% establishing the design goal first
% \thename establishes its objectives by introducing a novel \emph{hardware-enhanced capability model} that incorporates hardware security features of the recent and upcoming ARM architecture, whose principles and directions exhibit the characteristics of capability.
% In \thename's capability model, \thename domain is identified and authenticated through a per-domain and kernel-managed \gls{pa} key, called the \emph{domain authentication key}. 
% Upon entering a domain, \thename's in-kernel reference monitor switches the currently activating \gls{pa} key of the process to \emph{domain authentication key} of the target domain.
% \thename grants exclusivity of an object to its owner domain by signing the object references (described in detail in \cref{sec:design:objects}) with the domain authentication keys and authenticating the domain on use, thus creating \emph{capability tokens} that are only valid when the context is within their owner object.

% \added{
% \thename's coherent capability model protects sensitive program objects throughout their life cycles, from their import from the file system to their access through a file descriptor and finally to the access of their in-memory representation through a pointer.
% To this end, \thename identifies different types of sensitive resource references and, devises \gls{mte} and \gls{pa}-accelerated authentication policies that enable the simple yet effective isolation for each type of reference. 
% }
% The primary objectives of \thename are to guarantee exclusive access rights to private objects for each domain and to prevent a domain from escalating its privileges to access other domains' private objects.
% \thename's comprehensive and coherent capability model protects sensitive program objects throughout their life cycles. 
% This means that a private object is protected from its import from the file system to its access through a file descriptor, and finally to the access of its in-memory representation through a pointer.   




% \subsection{\added{Enforcement strategy}}

% \libcapac provides programmers with \thename API functions and also provides runtime facilities that are imperative to secure operations of other components.
% \thename's kernel-level reference monitor interposes system calls in of a \thename-enabled process to mediate all process file object creation and uses.

% \chcomment{mention something about annotation here}
% Our instrumentation framework \deleted{is built from scratch on top of LLVM 14.0.0~\cite{llvm} to} guarantees authenticated uses of all pointers through whole-program instrumentation. 
% It enforces \pamte-assisted domain memory isolation through managing domain-private tagged memory and \emph{domain-aware} pointer authentication.
% \autoref{tbl:objects} outlines the signing scheme for \thename references. 

% \deleted{
% \thename's design establishes intra-process isolation of file and memory objects through capability-based access control principles. 
% The design coherently incorporates hardware security features of the recent and upcoming ARM architecture, whose principles and directions exhibit the characteristics of capability.
% \thename's design demonstrates a comprehensive and capability-based \gls{ipi} model that can be applied to commodity ARM systems that support \gls{pa} and \gls{mte}. 
% }


==> tables/eval-applications.tex <==
\begin{table}
\footnotesize
 \begin{tabularx}{\columnwidth}{@{}lXcl@{}}
 \toprule
 \thead{Applications} & \thead{Isolated Objects \{Ref. Types\}}& \thead{No. of\\domains}& \thead{Modified\\SLOC} \\
 \midrule
 \makecell[l]{NGINX (v1.23.0)\\+LibreSSL (vx,x,x)} & \makecell[l]{Private key\{\cpath, \fd,\ptr\}\\TLS Session key\{\ptr\}\\Sokets \{\fd\}} & 3 \\
 \midrule
 OpenSSH (v1.1.1) & Private key \{\cpath, \fd,\ptr\} & 1 \\
 \midrule
 minizip &Password \{\ptr\}& 1\\
 \midrule
 wget (v1.1.1) & Password \{\ptr\}& 1\\

 
 \bottomrule
 \end{tabularx}

\caption{Programs used to evaluate \thename's resource isolation. }

\label{tbl:porting-app}
\label{tbl:app}
\end{table}
